Planning in Learned Latent Action Spaces for Generalizable Legged Locomotion

Hierarchical learning has been successful at learning generalizable locomotion skills on walking robots in a sample-efficient manner. However, the low-dimensional "latent" action used to communicate between two layers of the hierarchy is typically user-designed. In this work, we present a fully-learned hierarchical framework, that is capable of jointly learning the low-level controller and the high-level latent action space. Once this latent space is learned, we plan over continuous latent actions in a model-predictive control fashion, using a learned high-level dynamics model. This framework generalizes to multiple robots, and we present results on a Daisy hexapod simulation, A1 quadruped simulation, and Daisy robot hardware. We compare a range of learned hierarchical approaches from literature, and show that our framework outperforms baselines on multiple tasks and two simulations. In addition to learning approaches, we also compare to inverse-kinematics (IK) acting on desired robot motion, and show that our fully-learned framework outperforms IK in adverse settings on both A1 and Daisy simulations. On hardware, we show the Daisy hexapod achieve multiple locomotion tasks, in an unstructured outdoor setting, with only 2000 hardware samples, reinforcing the robustness and sample-efficiency of our approach.

==> comparison_table.tex <==
\begin{table}\centering
\scriptsize{
\ra{0.95}
\begin{tabular}{@{}llccc@{}}\toprule
& Method & $c_1$(\si{\meter/\second}) & $c_2$(\si{m/s}) & $c_3$(\si{m}) \\ \midrule
\multirow{3}{*}{Simulation} & LAT \scriptsize{(ours)} & $2.54 \pm 0.13$ & $\mathbf{8.26 \pm 0.66}$ & $\mathbf{152.54 \pm 13.97}$ \\
& FOOT & $2.73 \pm 0.10$ & $17.65 \pm 0.74$ & $175.15 \pm 7.58$ \\
& EXP & $\mathbf{2.38 \pm 0.02}$ & $14.13 \pm 0.30$ & $NA$ \\ \midrule

\multirow{3}{*}{Hardware} & LAT \scriptsize{(ours)} & $2.63 \pm 0.17$ & $\mathbf{11.96 \pm 0.40}$ & $194.56 \pm 19.41$ \\
& FOOT & $\mathbf{2.17 \pm 0.12}$ & $15.17 \pm 1.12$ & $\mathbf{166.20 \pm 9.29}$ \\
& EXP & $2.93 \pm 0.22$ & $12.05 \pm 0.41$ & $NA$ \\ \midrule
\end{tabular}
\caption{\small Simulation and hardware costs of different methods, over 5 runs in simulation and 3 runs on hardware. While footstep planning is better at tracking target speed ($c_1$), latent action planning reduced CoM accelerations and performs better at $c_2$. Latent space planning is better at trajectory tracking in simulation, but suffers on hardware due to simulation-hardware mismatch.}
\label{tab:compare}
}
\vspace{-0.3cm}
\end{table}
